Snowmass2021 Cosmic Frontier Dark Matter Direct Detection to the Neutrino Fog

We present a summary of future prospects for direct detection of dark matter within the GeV/c2 to TeV/c2 mass range. This is paired with a new definition of the neutrino fog in order to better quantify the rate of diminishing returns on sensitivity due to irreducible neutrino backgrounds. A survey of dark matter candidates predicted to fall within this mass range demonstrates that fully testing multiple well-motivated theo-ries will require expanding the currently-funded generation of experiments down to and past the neutrino fog. We end with the status and plans for next-generation exper-iments and novel R&D concepts which will get us there.

==> directionaldetection.tex <==
%I don't think this file is used. Remove? --Sven

%\subsubsection{Directional detectors}
%Current state of directional detectors. What proposals exist to scale-up %mass? 
%\begin{figure}
%    \centering
%    %\includegraphics{}
%    \missingfigure{Sensitivity of current and near-future directional %detectors}
%    \caption{Sensitivity of current and near-future directional detectors}
%    \label{fig:directional_sensitivity}
%end{figure}

==> eft.tex <==
\subsection{EFT couplings}
Lead: David Cerdeno

For the N most basic EFT couplings, What is the currently-excluded cross section from published results?  \textbf{Is there a mass range that is not being probed in one or more couplings?} Are there new technologies that uniquely address some portion of this parameter space?

\begin{figure}
    \centering
    %\includegraphics{}
    \missingfigure[figheight=16cm]{EFT cross section space excluded}
    \caption{7 or so plots of current and near-future EFT cross-section sensitivity.}
    \label{fig:EFT_sensitivity}
\end{figure}


% Prisca: I suppose our charge is to the neutrino floor. Are ER searches the only thing getting there (under our charge)?   Do we cover only electron scattering (elastic and inelastic) and NOT dark sector stuff and dark photon absorption?   What about getting to the neutrino floor at low mass? This is kind of interesting, because the neutrino floor focus could move the discussion away from pushing to the lowest threshold and open up and interesting examination of what the real limit is to low mass at the largest exposures. Thus, a better organizational principle might be for mass regions instead of NR vs ER.  The theory might be easier to subdivide, too.   But if not, I tried to subdivide ER without low mass. 

==> experiments/darwin.tex <==
DARWIN Lead:


